Cross-Representation Benchmarking in Time-Series Electronic Health Records for Clinical Outcome Prediction

Electronic Health Records (EHRs) enable deep learning for clinical predictions, but the optimal method for representing patient data remains unclear due to inconsistent evaluation practices. We present the first systematic benchmark to compare EHR representation methods, including multivariate time-series, event streams, and textual event streams for LLMs. This benchmark standardises data curation and evaluation across two distinct clinical settings: the MIMIC-IV dataset for ICU tasks (mortality, phenotyping) and the EHRSHOT dataset for longitudinal care (30-day readmission, 1-year pancreatic cancer). For each paradigm, we evaluate appropriate modelling families--including Transformers, MLP, LSTMs and Retain for time-series, CLMBR and count-based models for event streams, 8-20B LLMs for textual streams--and analyse the impact of feature pruning based on data missingness. Our experiments reveal that event stream models consistently deliver the strongest performance. Pre-trained models like CLMBR are highly sample-efficient in few-shot settings, though simpler count-based models can be competitive given sufficient data. Furthermore, we find that feature selection strategies must be adapted to the clinical setting: pruning sparse features improves ICU predictions, while retaining them is critical for longitudinal tasks. Our results, enabled by a unified and reproducible pipeline, provide practical guidance for selecting EHR representations based on the clinical context and data regime.

==> combined_with_intro-related_works.tex <==
% \section{Related Work}
% \label{sec:related_work}

% \subsection{ICU Outcome Prediction Benchmarks}  
% Benchmarks based on the EHR databases have played a central role in evaluating machine learning for ICU outcome prediction. Specifically, \citeauthor{harutyunyan2019multitask}~\cite{harutyunyan2019multitask} curated the EHR as multivariate time-series data and defined multiple clinical prediction tasks. Similarly, \citeauthor{gupta2022extensive}~\cite{gupta2022extensive} standardised feature extraction, outlier handling, and imputation strategies for the latest EHR datasets. While these benchmarks established common ground for model evaluation, they remain largely confined to regular time-series representations, overlooking alternative formulations of EHR data.  

% \subsection{Representation Methods for EHR Benchmarks}  
% Beyond multivariate time series, recent work explores event streams and textual representations as alternative ways to model EHR. Event streams preserve the original sequence of irregularly timed events, avoiding information loss from aggregation and imputation~\cite{arnrich2024medical, wornow2023ehrshot}. This representation has supported the development of foundation models such as CLMBR, which leverage large-scale pretraining for transferability across tasks. More recently, textualisation strategies serialise event streams into pseudo-clinical notes for direct use with large language models (LLMs)~\cite{lee2025clinical, battula2024enhancing}, enabling the integration of structured EHR with advances in natural language processing. These complementary representations—time series, event streams, and textual narratives—highlight a growing need for benchmarks that systematically compare their strengths and limitations on shared prediction tasks.  


% % \subsection{ICU Outcome Prediction Benchmarks}
% % The MIMIC-III database~\cite{johnson2016mimic} enabled several benchmark tasks for ICU stays. Harutyunyan et al.~\cite{harutyunyan2019multitask} defined four canonical tasks (mortality, length of stay, physiologic decompensation, and phenotype classification) and released preprocessing code to extract multivariate time-series features from ICU records. Based on this, recent work has begun to standardize MIMIC-IV preprocessing and evaluation. Researchers used a regular time-series representation with hourly sampled measurements and imputations, combined with simple baselines (logistic regression) and deep models (LSTM)~\cite{harutyunyan2019multitask, song2018attend}. Gupta et al.~\cite{gupta2022extensive} released a MIMIC-IV pipeline that extracts ICU cohorts and produces similar multivariate multivariate time series with clinical grouping, outlier handling, and imputation (forward-fill and mean) at a 2-hour resolution.  However, all these studies relied on a multivariate matrix representation of patient data. Our work extends this line by comparing that traditional representation with alternative forms.

% % \subsection{Event Stream Representation}
% % Rather than imposing a regular grid, another approach is to feed the model the sequence of events as they occurred, with each event carrying a timestamp, event type (code), and value. Event-stream modeling can naturally handle irregular timing and high dimensionality of codes. RETAIN~\cite{choi2016retain} is an example of an RNN-based model that processes a sequence of medical events with attention to provide interpretable predictions (it was originally applied to billing code sequences for heart failure prediction). More recently, the concept of pretrained foundation models on structured EHR data has emerged. Wornow et al.~\cite{wornow2023ehrshot} introduced EHRSHOT, a large EHR dataset (6.7k patients, 41M events) with 15 prediction tasks, along with CLMBR, a 141M-parameter Transformer pre-trained on 2.57M patients’ EHR data. CLMBR (Clinical Language Model for Binary Representation) is trained via causally masked next-event prediction on sequences of coded events, and has been shown to adapt well to new tasks with limited data. While EHRSHOT is more general (not limited to ICU stays), it uses a similar event-stream format that we adopt in our experiments. Prior studies have also explored transforming tabular MIMIC-IV into "pseudo-notes", a text serialization on EHR data, then used on language foundation models~\cite{lee2025clinical}. We will leverage the same iead of textual serialization of event streams combined with the use of LLM.


% % \subsection{Textualization of EHR for LLMs}
% % With the rise of large language models (LLMs), there is interest in transforming structured EHR data (event streams) into text that an LLM can process. Besides~\cite{lee2025clinical}, another emerging idea is prompting or fine-tuning LLMs to predict outcomes from a textual summary of a patient’s record~\cite{battula2024enhancing}. 
% % For example, recent work has used GPT-based models on patient narratives or combined clinical notes with structured data to improve mortality prediction[12]. 
% % Pushing toward structure-aware prompting, recent work encodes longitudinal EHR specifics (units, ranges, temporal context) and demonstrates zero- or few-shot improvements on MIMIC-IV tasks, emphasizing prompt engineering as a representation layer~\cite{zhu2024prompting}.
% % These approaches leverage the powerful reasoning and generalization abilities of LLMs, but challenges include how to faithfully encode all crucial numeric data into text and how to obtain calibrated probabilities for evaluation metrics like AUROC. 






==> scripts.tex <==

\subsection{ICU outcome prediction benchmarks on MIMIC-IV}
Beyond the widely used MIMIC-III benchmarks (hourly resampling with imputation; logistic regression and LSTM baselines)~\cite{harutyunyan2019multitask},  Building on this pipeline, Bui et al.~\cite{} benchmarked XGBoost, LSTM, and TCN on MIMIC-IV and reported that XGBoost can outperform deep models for mortality/LOS while still using fixed windows with imputation—again, a discretized-and-imputed representation rather than an event sequence. 

Complementary overview work emphasizes that most ICU benchmarking still relies on preprocessed tabular time series (demographics, labs, vitals), with missingness handled via imputation and masks, and only a minority of studies incorporate clinical notes or alternate encodings. In parallel, several \emph{method} papers target \textbf{irregular-sampling} directly—e.g., HeTVAE/UnTAN (uncertainty-aware attention over reference times), ODE-RNN (continuous-time latent dynamics), GRU-D/T-LSTM (time-aware RNNs), and STRaTS (treating data as \emph{triplets} of \{time, variable, value\} with continuous value embeddings)—which move closer to \emph{event-stream} modeling but have not yet coalesced into a standardized MIMIC-IV benchmark protocol. :contentReference[oaicite:5]{index=5} :contentReference[oaicite:6]{index=6} 

Finally, recent MIMIC-IV ``textualization'' efforts still \emph{start} from the regularized tabular pipeline (fixed windows + imputation) and then convert features to templated narratives for LLMs, reinforcing that the dominant benchmark data layer in MIMIC-IV remains a \textbf{regular time-grid matrix} rather than raw event streams. :contentReference[oaicite:7]{index=7}


methodology?

In this work, we convert MIMIC-IV ICU data into the OMOP standardized coding used by CLMBR, allowing us to leverage the released CLMBR model as a feature extractor or fine-tuned model on our tasks. We also evaluate a simpler count-based representation as a baseline, where each patient’s record is summarized by counts or frequencies of different event codes (an approach used in EHRSHOT benchmarks via a Gradient Boosted Trees model). 

In our study, we include a preliminary exploration of an LLM-based approach: we convert each patient’s ICU stay into a textual description of events (vitals, labs, etc.) and prompt an LLM to classify outcomes. This allows us to compare its performance (using F1-score) to the structured representations, acknowledging that direct AUROC/AUPRC comparison is not straightforward for generative LLM outputs.

In contrast to note-only or template-summary pipelines, we textualize the structured EHR into an ordered event stream—each tokenized entry is \texttt{(time, code, value)} using OMOP/LOINC/RxNorm and preserved chronology—so the LLM reasons directly over temporality and coded measurements rather than over imputed grids or clinician-authored narratives.

==> table2.tex <==

\begin{table*}[htbp]
\centering
\caption{Model Performance on 30-day Readmission Prediction with Varying Data Rates on EHRSHOT}
\label{tab:readmission_performance}
\resizebox{\textwidth}{!}{%
\begin{tabular}{llccccccc}
\toprule
\textbf{Data Rate} & \textbf{Model} & \textbf{Val AUPRC} & \textbf{Val AUROC} & \textbf{Test AUPRC} & \textbf{Test AUROC} & \textbf{F1 (best)} & \textbf{F1 @ 0.5} & \textbf{Thr (best)} \\
\midrule
\multirow{4}{*}{90.0\%} & transformer & 0.2143 & 0.6512 & 0.1886 & 0.6516 & 0.2893 & 0.2698 & 0.708 \\
 & lstm & 0.2165 & 0.6438 & 0.1710 & 0.6414 & 0.2733 & 0.2649 & 0.526 \\
 & retain & 0.1773 & 0.6199 & 0.1581 & 0.6125 & 0.2435 & 0.2250 & 0.471 \\
 & mlp & 0.2196 & 0.6639 & 0.1522 & 0.6191 & 0.2599 & 0.2533 & 0.481 \\
\midrule
\multirow{4}{*}{92.5\%} & mlp & 0.2430 & 0.6778 & 0.2018 & 0.6589 & 0.2895 & 0.2582 & 0.595 \\
 & retain & 0.2235 & 0.6481 & 0.1861 & 0.6630 & 0.2839 & 0.2750 & 0.594 \\
 & lstm & 0.2254 & 0.6558 & 0.1859 & 0.6720 & 0.2944 & 0.2757 & 0.621 \\
 & transformer & 0.1725 & 0.6006 & 0.1556 & 0.5970 & 0.2759 & 0.2095 & 0.605 \\
\midrule
\multirow{4}{*}{95.0\%} & retain & 0.2251 & 0.6462 & 0.2013 & 0.6516 & 0.2742 & 0.2635 & 0.470 \\
 & mlp & 0.2581 & 0.6890 & 0.1915 & 0.6568 & 0.2734 & 0.2674 & 0.619 \\
 & lstm & 0.2373 & 0.6583 & 0.1882 & 0.6574 & 0.2765 & 0.2666 & 0.609 \\
 & transformer & 0.1927 & 0.6288 & 0.1667 & 0.6109 & 0.2565 & 0.2395 & 0.620 \\
\midrule
\multirow{5}{*}{97.5\%} & lstm & 0.2704 & 0.6571 & 0.2525 & 0.6739 & 0.2829 & 0.2593 & 0.665 \\
 & mlp & 0.2660 & 0.6763 & 0.2332 & 0.6821 & 0.3171 & 0.2754 & 0.609 \\
 & transformer & 0.2480 & 0.6540 & 0.2253 & 0.6781 & 0.3032 & 0.0000 & 0.484 \\
 & retain & 0.2547 & 0.6522 & 0.2193 & 0.6827 & 0.3200 & 0.2957 & 0.543 \\
 & transformer & 0.2128 & 0.6339 & 0.1785 & 0.6406 & 0.2633 & 0.2091 & 0.622 \\
\midrule
\multirow{4}{*}{100.0\%} & lstm & 0.3074 & 0.7237 & 0.3180 & 0.7603 & 0.3827 & 0.3761 & 0.570 \\
 & retain & 0.2993 & 0.7202 & 0.3143 & 0.7573 & 0.3893 & 0.3820 & 0.517 \\
 & mlp & 0.2685 & 0.6983 & 0.2930 & 0.7633 & 0.3858 & 0.3409 & 0.567 \\
 & transformer & 0.2496 & 0.6860 & 0.2604 & 0.7430 & 0.3822 & 0.2040 & 0.538 \\
\bottomrule
\end{tabular}%
}
\end{table*}




\begin{table*}[ht]
\centering
\caption{Performance comparison on the Pancreatic Cancer prediction task under different feature missing rate thresholds. The best result for each metric is highlighted in \textbf{bold}.}
\label{tab:pancan_results}
\begin{tabular}{llccc}
\toprule
\textbf{Missing Rate} & \textbf{Model} & \textbf{Test AUROC} & \textbf{Test AUPRC} & \textbf{F1 (best)} \\
\textbf{Threshold} & & & & \\
\midrule
\multirow{4}{*}{90.0\%} 
& MLP & 0.645 & 0.049 & 0.125 \\
& LSTM & 0.614 & 0.045 & 0.103 \\
& RETAIN & 0.615 & 0.042 & 0.095 \\
& Transformer & 0.516 & 0.035 & 0.079 \\
\midrule
\multirow{4}{*}{92.5\%} 
& MLP & 0.643 & 0.067 & 0.129 \\
& Transformer & 0.614 & 0.052 & 0.099 \\
& LSTM & 0.603 & 0.052 & 0.103 \\
& RETAIN & 0.641 & 0.050 & 0.093 \\
\midrule
\multirow{4}{*}{95.0\%} 
& MLP & 0.659 & 0.069 & 0.149 \\
& LSTM & 0.633 & 0.040 & 0.099 \\
& Transformer & 0.608 & 0.039 & 0.098 \\
& RETAIN & 0.553 & 0.034 & 0.080 \\
\midrule
\multirow{4}{*}{97.5\%} 
& MLP & 0.540 & 0.037 & 0.080 \\
& LSTM & 0.601 & 0.031 & 0.072 \\
& RETAIN & 0.512 & 0.028 & 0.067 \\
& Transformer & 0.535 & 0.027 & 0.059 \\
\midrule
\multirow{4}{*}{\parbox{2.5cm}{\raggedright 100\% \\ (No Filtering)}} 
& LSTM & \textbf{0.739} & \textbf{0.148} & \textbf{0.222} \\
& RETAIN & 0.688 & 0.117 & \textbf{0.222} \\
& MLP & 0.716 & 0.106 & 0.202 \\
& Transformer & 0.588 & 0.038 & 0.083 \\
\bottomrule
\end{tabular}
\end{table*}

\begin{table*}[ht]
\centering
\caption{Model performance on ICU mortality prediction with different levels of feature filtering based on missingness. The best result for each metric across all experiments is in \textbf{bold}.}
\label{tab:feature_selection_results}
\begin{tabular}{clccc}
\toprule
\textbf{Kept} & \textbf{Model} & \textbf{Test AUROC} & \textbf{Test AUPRC} & \textbf{F1 (best)} \\
\textbf{Features} & & & & \\
\midrule
\multirow{4}{*}{802} 
& MLP & 0.857 & 0.367 & 0.418 \\
& RETAIN & 0.858 & 0.340 & 0.424 \\
& LSTM & 0.808 & 0.300 & 0.354 \\
& Transformer & 0.726 & 0.225 & 0.322 \\
\midrule
\multirow{4}{*}{89} 
& LSTM & \textbf{0.869} & \textbf{0.401} & 0.432 \\
& MLP & 0.862 & 0.380 & 0.430 \\
& RETAIN & 0.863 & 0.369 & \textbf{0.439} \\
& Transformer & 0.803 & 0.264 & 0.342 \\
\midrule
\multirow{4}{*}{70} 
& LSTM & 0.869 & 0.389 & 0.433 \\
& MLP & 0.862 & 0.365 & 0.438 \\
& RETAIN & 0.857 & 0.350 & 0.405 \\
& Transformer & 0.708 & 0.181 & 0.315 \\
\midrule
\multirow{4}{*}{58} 
& MLP & 0.855 & 0.385 & 0.421 \\
& LSTM & 0.856 & 0.376 & 0.416 \\
& RETAIN & 0.847 & 0.347 & 0.411 \\
& Transformer & 0.638 & 0.146 & 0.263 \\
\midrule
\multirow{4}{*}{23} 
& RETAIN & 0.798 & 0.302 & 0.353 \\
& LSTM & 0.810 & 0.300 & 0.349 \\
& MLP & 0.794 & 0.272 & 0.310 \\
& Transformer & 0.575 & 0.106 & 0.216 \\
\midrule
\multirow{4}{*}{7} 
& RETAIN & 0.745 & 0.207 & 0.263 \\
& LSTM & 0.763 & 0.205 & 0.276 \\
& MLP & 0.747 & 0.204 & 0.291 \\
& Transformer & 0.557 & 0.076 & 0.147 \\
\bottomrule
\end{tabular}
\end{table*}
